On Weighted Graph Sparsification by Linear Sketching

A seminal work of [Ahn-Guha-McGregor, PODS'12] showed that one can compute a cut sparsifier of an unweighted undirected graph by taking a near-linear number of linear measurements on the graph. Subsequent works also studied computing other graph sparsifiers using linear sketching, and obtained near-linear upper bounds for spectral sparsifiers [Kapralov-Lee-Musco-Musco-Sidford, FOCS'14] and first non-trivial upper bounds for spanners [Filtser-Kapralov-Nouri, SODA'21]. All these linear sketching algorithms, however, only work on unweighted graphs. In this paper, we initiate the study of weighted graph sparsification by linear sketching by investigating a natural class of linear sketches that we call incidence sketches, in which each measurement is a linear combination of the weights of edges incident on a single vertex. Our results are: 1. Weighted cut sparsification: We give an algorithm that computes a $(1 + \epsilon)$-cut sparsifier using $\tilde{O}(n \epsilon^{-3})$ linear measurements, which is nearly optimal. 2. Weighted spectral sparsification: We give an algorithm that computes a $(1 + \epsilon)$-spectral sparsifier using $\tilde{O}(n^{6/5} \epsilon^{-4})$ linear measurements. Complementing our algorithm, we then prove a superlinear lower bound of $\Omega(n^{21/20-o(1)})$ measurements for computing some $O(1)$-spectral sparsifier using incidence sketches. 3. Weighted spanner computation: We focus on graphs whose largest/smallest edge weights differ by an $O(1)$ factor, and prove that, for incidence sketches, the upper bounds obtained by~[Filtser-Kapralov-Nouri, SODA'21] are optimal up to an $n^{o(1)}$ factor.

==> headers.tex <==
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{shapes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{patterns}
\usetikzlibrary{calc}
\usetikzlibrary{fit}
\usetikzlibrary{snakes}
\usetikzlibrary{shadows.blur}
\usetikzlibrary{petri,decorations.markings}

\renewcommand{\top}{T}

\RequirePackage{silence}
\WarningFilter{remreset}{The remreset package}
\usepackage{fancybox}
\usepackage{enumitem}

\setlistdepth{9}

\newlist{myEnumerate}{enumerate}{5}
\setlist[myEnumerate,1]{label=\arabic*.}
\setlist[myEnumerate,2]{label=(\alph*)}
\setlist[myEnumerate,3]{label=\roman*.}
\setlist[myEnumerate,4]{label=\Alph*.}
\setlist[myEnumerate,5]{label=\Roman*.}

\usepackage{kbordermatrix}
\renewcommand{\kbldelim}{(}%
\renewcommand{\kbrdelim}{)}%
\usepackage{blkarray}
\usepackage{array}
\newcolumntype{x}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\mLabel}[1]{\mbox{$\scriptstyle{#1}$}}

\usepackage{stackengine}
\newcommand\xrowht[2][0]{\addstackgap[.5\dimexpr#2\relax]{\vphantom{#1}}}

\newcommand{\gy}{G_{\sigma_n}^{\mathrm{yes}}}
\newcommand{\gn}{G_{\sigma_n}^{\mathrm{no}}}
\newcommand{\dtv}{D_{\mathrm{TV}}}

\usepackage{amsmath,amsfonts,amssymb,amsthm,bm}
\usepackage{color,xcolor}
\usepackage[colorlinks=true]{hyperref}
\usepackage[procnumbered,ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{amsfonts}
\usepackage{thm-restate}
\usepackage{blindtext}
\usepackage{thm-restate}

\textheight 8.5in
\topmargin -0.2in
\oddsidemargin 0.20in
\textwidth 6.3in

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemm}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{assumption}[lemm]{Assumption}
\newtheorem{definition}[lemm]{Definition}
\newtheorem{remark}[lemm]{Remark}
\newtheorem{problem}{Problem}


\newcommand{\highlight}[1]{\colorbox{yellow}{#1}}


\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}

\newenvironment{algbox}[0]{%
\noindent
  \begin{center}
\begin{fminipage}{1\textwidth}%
}{
\end{fminipage}
\end{center}
}


\DontPrintSemicolon
\SetKw{KwAnd}{and}
\SetProcNameSty{textsc}
\SetFuncSty{textsc}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\def\dr{\mathrm{d}}

\def\pleq{\preceq} %
\def\pgeq{\succeq} %
\def\pge{\succ}
\def\ple{\prec}
\def\sc{\textsc{SC}}

\newcommand\AGM{\textsc{UnweightedCutSparsify}}
\newcommand\WGM{\textsc{WeightedCutSparsify}}
\newcommand\WL{\textsc{WeightedEdgeSampler}}

\newcommand\HVS{\textsc{HeavyEdgeSketch}}
\newcommand\HVR{\textsc{HeavyEdgeRecovery}}

\newcommand\WSS{\textsc{SpectralSketch}}
\newcommand\WSR{\textsc{SpectralRecovery}}

\newcommand\SQS{\textsc{SquareSketch}}
\newcommand\SQR{\textsc{SquareRecovery}}

\newcommand\SVS{\textsc{SquareHeavySketch}}
\newcommand\SVR{\textsc{SquareHeavyRecovery}}

\newcommand\SSQ{S^{\mathrm{sq}}}
\newcommand\SSS{S^{\mathrm{ss}}}
\newcommand\SHV{S^{\mathrm{hv}}}
\newcommand\SSV{S^{\mathrm{sqh}}}

\def\detp{\det\nolimits_{+}}
\def\detb#1{\det\nolimits_{#1}}
\def\detz{\det\nolimits_{(0,\zeta]}}
\def\detzz{\det\nolimits_{(0,\zeta']}}
\def\detl{\det\nolimits_{\ell}}
\def\detll{\det\nolimits_{\ell'}}
\def\detn{\det\nolimits}

\def\dr{\mathrm{d}}

\def\Approx#1{\approx_{#1}}

\def\Span#1{\textbf{Span}\left(#1  \right)}
\def\bvec#1{{\mbox{\boldmath $#1$}}}


\def\prob#1#2{\mathrm{Pr}_{#1}\left[ #2 \right]}
\def\pr#1{\mathrm{Pr}\left[ #1 \right]}
\def\pvec#1#2{\vec{\mbox{P}}^{#1}\left[ #2 \right]}
\def\expec#1#2{{\mathbb{E}}_{#1}\left[ #2 \right]}
\def\ex#1{{\mathbb{E}}\left[ #1 \right]}
\def\var#1{\mbox{\bf Var}\left[ #1 \right]}
\newcommand{\E}{\mbox{{\bf E}}}

\def\defeq{\stackrel{\mathrm{def}}{=}}
\def\setof#1{\left\{#1  \right\}}
\def\sizeof#1{\left|#1  \right|}
\def\deg{\textrm{deg}}




\def\floor#1{\left\lfloor #1 \right\rfloor}
\def\ceil#1{\left\lceil #1 \right\rceil}

\def\dim#1{\mathrm{dim} (#1)}
\def\sgn#1{\mathrm{sgn} (#1)}

\def\union{\cup}
\def\intersect{\cap}
\def\Union{\bigcup}
\def\Intersect{\bigcap}

\def\eps{\epsilon}

\def\abs#1{\left|#1  \right|}

\def\rank#1{\mathrm{rank} \left(#1 \right)}
\def\trace#1{\mathrm{Tr} \left(#1 \right)}
\def\norm#1{\left\| #1 \right\|}
\def\normm#1{\lambdamax\kh{#1}}
\def\smallnorm#1{\| #1 \|}

\def\comp#1{#1^\complement}

\def\Acal{\mathcal{A}}
\def\Ncal{\mathcal{N}}
\def\Rcal{\mathcal{R}}
\def\Bcal{\mathcal{B}}
\def\Ccal{\mathcal{C}}
\def\Dcal{\mathcal{D}}
\def\Ecal{\mathcal{E}}
\def\Fcal{\mathcal{F}}
\def\Mcal{\mathcal{M}}
\def\Xcal{\mathcal{X}}
\def\Ftil{\tilde{F}}
\def\Htil{\tilde{H}}
\def\Ztil{\tilde{Z}}
\def\Ltil{\tilde{L}}
\def\wtil{\tilde{w}}
\def\Fcaltil{\tilde{\mathcal{F}}}
\def\Lambdatil{\tilde{\Lambda}}
\def\Hcal{\mathcal{H}}
\def\Ical{\mathcal{I}}
\def\Itil{\tilde{{I}}}
\def\Gcal{\mathcal{G}}
\def\Rcal{\mathcal{R}}
\def\phitil{\tilde{\phi}}
\def\Ucal{\mathcal{U}}
\def\Vcal{\mathcal{V}}
\def\Lcal{\mathcal{L}}
\def\Scal{\mathcal{S}}
\newcommand\Tcal{\mathcal{T}}
\newcommand\Pcal{\mathcal{P}}

\newcommand\xtil{\tilde{x}}
\newcommand\Gtil{\tilde{G}}

\newcommand\pth{\mathfrak{p}}


\newcommand\Ppsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\PPsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\ppsi{\boldsymbol{\mathit{\psi}}}
\newcommand\pphi{\boldsymbol{\mathit{\phi}}}
\newcommand\Llambda{\boldsymbol{\mathit{\Lambda}}}
\newcommand\PPi{\boldsymbol{\Pi}}

\newcommand\ppi{\vec{\pi}}
\newcommand\cchi{\boldsymbol{\chi}}
\newcommand\aalpha{\boldsymbol{\alpha}}
\newcommand\bbeta{\boldsymbol{\beta}}
\newcommand\ggamma{\boldsymbol{\gamma}}
\newcommand\ddelta{\boldsymbol{\delta}}

\newcommand\er{R_{\mathrm{eff}}}
\newcommand\ccc{C_{\mathrm{CC}}}
\newcommand\ci{C_{\mathrm{I}}}


\def\lev{\mathtt{lev}}
\def\aa{\pmb{\mathit{a}}}
\newcommand\bb{\boldsymbol{\mathit{b}}}
\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\dd{\boldsymbol{\mathit{d}}}
\newcommand\ee{\boldsymbol{\mathit{e}}}
\newcommand\ff{\boldsymbol{\mathit{f}}}
\newcommand\ii{\boldsymbol{\mathit{i}}}
\newcommand\jj{\boldsymbol{\mathit{j}}}
\newcommand\kk{\boldsymbol{\mathit{k}}}
\newcommand\pp{\boldsymbol{\mathit{p}}}
\newcommand{\ttau}{{\boldsymbol{\mathit{\tau}}}}
\newcommand\qq{\boldsymbol{\mathit{q}}}
\newcommand\bs{\boldsymbol{\mathit{s}}}
\newcommand\nn{\vec{n}}
\newcommand\mm{\vec{m}}
\newcommand\rr{\boldsymbol{\mathit{r}}}
\newcommand\rrh{{\boldsymbol{\widehat{\mathit{{r}}}}}}
\renewcommand\dh{\widehat{d}}
\newcommand\wh{\widehat{w}}
\renewcommand\ss{\boldsymbol{\mathit{s}}}
\def\tt{\boldsymbol{\mathit{t}}}
\newcommand\uu{\boldsymbol{\mathit{u}}}
\newcommand\vv{\boldsymbol{\mathit{v}}}
\newcommand\ww{\boldsymbol{\mathit{w}}}
\newcommand\yy{\boldsymbol{\mathit{y}}}
\newcommand\zz{\boldsymbol{\mathit{z}}}
\newcommand\xx{\boldsymbol{\mathit{x}}}
\newcommand\xxbar{\overline{\boldsymbol{\mathit{x}}}}

\newcommand\dbar{d_{\mathrm{avg}}}

\renewcommand\AA{\boldsymbol{\mathit{A}}}
\newcommand\BB{\boldsymbol{\mathit{B}}}
\newcommand\CC{\boldsymbol{\mathit{C}}}
\newcommand\DD{\boldsymbol{\mathit{D}}}
\newcommand\EE{\boldsymbol{\mathit{E}}}
\newcommand\GG{\boldsymbol{\mathit{G}}}
\newcommand\II{\boldsymbol{\mathit{I}}}
\newcommand\JJ{\boldsymbol{\mathit{J}}}
\newcommand\KK{\boldsymbol{\mathit{K}}}
\newcommand\NN{\boldsymbol{\mathit{N}}}
\newcommand\MM{\mathrm{\textsf{M}}}
\newcommand\LL{\boldsymbol{\mathit{L}}}
\newcommand\HH{\boldsymbol{\mathit{H}}}
\newcommand\PP{\boldsymbol{\mathit{P}}}
\newcommand\QQ{\boldsymbol{\mathit{Q}}}
\newcommand\RR{\boldsymbol{\mathit{R}}}
\renewcommand\SS{\boldsymbol{\mathit{S}}}
\newcommand\TT{\boldsymbol{\mathit{T}}}
\newcommand\UU{\boldsymbol{\mathit{U}}}
\newcommand\WW{\boldsymbol{\mathit{W}}}
\newcommand\VV{\boldsymbol{\mathit{V}}}
\newcommand\XX{\boldsymbol{\mathit{X}}}
\newcommand\YY{\boldsymbol{\mathit{Y}}}

\def\sfy{{\sf Yes} }
\def\sfn{{\sf No} }
\newcommand\nnz{\mathrm{nnz}}
\newcommand\tv{\mathrm{TV}}
\newcommand\yes{\mathrm{yes}} %
\newcommand\no{\mathrm{no}}

\newcommand\shat{\hat{s}}
\newcommand\ftil{\tilde{f}}
\newcommand\lambdatil{\tilde{\lambda}}
\newcommand\Ntil{\tilde{N}}
\newcommand\dtil{\tilde{d}}
\newcommand\Dtil{\tilde{D}}
\newcommand\MMtil{\boldsymbol{\mathit{\tilde{M}}}}
\newcommand\AAtilde{\boldsymbol{\mathit{\tilde{A}}}}
\newcommand\LLtil{\boldsymbol{\mathit{\tilde{L}}}}
\newcommand\MMtilde{\boldsymbol{\mathit{\tilde{M}}}}

\newcommand\AAn{\boldsymbol{\mathcal{A}}}
\newcommand\ZZ{\boldsymbol{\mathit{Z}}}

\newcommand\ZZtil{\widetilde{\boldsymbol{\mathit{Z}}}}

\newcommand\AAhat{\boldsymbol{\widehat{\mathit{A}}}}
\newcommand\AAapprox{\boldsymbol{\widetilde{\mathit{A}}}}
\newcommand\DDhat{\boldsymbol{\widehat{\mathit{D}}}}
\newcommand\DDapprox{\boldsymbol{\widetilde{\mathit{D}}}}
\newcommand\LLhat{\boldsymbol{\widehat{\mathit{L}}}}
\newcommand\LLapprox{\boldsymbol{\widetilde{\mathit{L}}}}
\newcommand\MMhat{\boldsymbol{\widehat{\mathit{M}}}}
\newcommand\MMapprox{\boldsymbol{\widetilde{\mathit{M}}}}
\newcommand\ZZhat{\boldsymbol{\widehat{\mathit{Z}}}}

\newcommand\AAtil{\boldsymbol{\widetilde{\mathit{A}}}}
\newcommand\DDtil{\boldsymbol{\widetilde{\mathit{D}}}}


\newcommand\bbtil{\boldsymbol{\tilde{\mathit{b}}}}
\newcommand\xxtil{\boldsymbol{\tilde{\mathit{x}}}}


\newcommand\Otil{\tilde{O}}
\newcommand\otil{\tilde{o}}
\newcommand\Ktil{\tilde{K}}
\newcommand\Thetatil{\tilde{\Theta}}
\newcommand\Omegatil{\tilde{\Omega}}

\newcommand\xhat{\boldsymbol{\hat{\mathit{x}}}}
\newcommand\uhat{{\hat{{u}}}}
\newcommand\vhat{{\hat{{v}}}}
\newcommand\what{{\hat{{w}}}}

\newcommand\fbf{\mathbf{f}}

\newcommand\Ghat{{\widehat{{G}}}}

\newcommand{\sym}[1]{\mathrm{sym} (#1)}

\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\diag}{\textsc{diag}}
\newcommand\LLs{\boldsymbol{\mathit{L}_s}}
\newcommand\SSi{\boldsymbol{\Sigma}}

\newcommand\dila{\mathtt{dila}}
\newcommand\cont{\mathtt{ctrc}}
\newcommand\area{\mathtt{area}}
\newcommand\vol{\mathrm{vol}}
\newcommand\scolon{\hspace{-2.5pt}:\hspace{-1.5pt}}

\newcommand\DS{\textsc{DetScheduling}}
\newcommand\DP{\textsc{DPScheduling}}
\newcommand\RI{\textsc{Rounded}}
\newcommand\PTAS{\textsc{PoiScheduling}}
\newcommand\ILP{\textsc{ILPScheduling}}
\newcommand\IP{\textsc{ILP}}
\newcommand\CHEBY{\textsc{ChebySolve}}
\newcommand\HARGD{\textsc{AlmostRegularDecomp}}
\newcommand\HED{\textsc{ExpanderDecomp}}
\newcommand\WAM{\textsc{Whack-a-mole-I}}
\newcommand\WTM{\textsc{Whack-a-mole-II}}
\newcommand\WAME{\textsc{Whack-a-mole-Exp}}

\newcommand\la{\leftarrow}

\newcommand\TEST{\textsc{Traps?}}
\newcommand\MBSWB{\textsc{NoisyBinarySearchRW}}

\newcommand\IR{\textsc{Sparisfy}}
\newcommand\SP{\textsc{SampleWR}}

\newcommand\SC{\mathrm{SC}}
\newcommand\SCN{\mathrm{SC}_n}

\newcommand{\sd}{\geq_{\mathrm{sd}}}

\newcommand{\todo}[1]{{\bf \color{red} TODO: #1}}
\newcommand{\hl}[1]{{\bf \color{orange} Huan: #1}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\poi}[1]{\mathrm{Poi}\left(#1\right)}

\newcommand{\kh}[1]{\left(#1\right)}

\newcommand{\ip}[2]{\left\langle#1,#2\right\rangle}

\newcommand{\wmax}{w_{\max}}
\newcommand{\wmin}{w_{\min}}

\newcommand{\lambdamin}{\lambda_{\mathrm{min}}}
\newcommand{\lambdamax}{\lambda_{\mathrm{max}}}

\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\ade}[1]{{\color{blue}#1}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\by}{\mathbf{y}}

\newcommand{\dmin}{d_{\mathrm{min}}}

